Matroids arising from electrical networks

This paper introduces Dirichlet matroids, a generalization of graphic matroids arising from electrical networks. We present four main theorems. First, we exhibit a matroid quotient involving geometric duals of networks embedded in surfaces with boundary. Second, we characterize the Bergman fans of Dirichlet matroids as subfans of graphic Bergman fans. Third, we prove an interlacing result on the real zeros and poles of the trace of the response matrix. And fourth, we bound the coefficients of the precoloring polynomial of a network by the coefficients of the associated chromatic polynomial.

==> sections/conn.tex <==
\section{3-Connectedness}
\label{mat:sec:conn}

We prove Theorem \ref{mat:thm:3connintro}. Our main tools are characterizations by Slilaty and Qin \cite{slilaty2008} of 2- and 3-connected bias matroids $G(\bg)$ in terms of the biased graph $\bg$. Given a biased graph $\bg$ we write $E(\bg)$ for the edge set of $\bg$.

\begin{mydef}
	For any integer $k\geq 1$, a \emph{vertical $k$-biseparation} of a biased graph $\bg = (\g,\BB)$ is a partition $(X,Y)$ of $E(\bg)$ satisfying the following two conditions:
	\begin{enumerate}[(i)]
		\item $|X|,|Y|\geq k$
		\item Each of $X$ and $Y$ meets a vertex not met by the other,
	\end{enumerate}
	and any one of the following three conditions:
	\begin{enumerate}[(i)]
		\setcounter{enumi}{2}
		\item $\ell = k+1$ with both $X$ and $Y$ balanced
		\item $\ell = k$ with only one of $X$ and $Y$ balanced
		\item $\ell = k-1$ with neither $X$ nor $Y$ balanced,
	\end{enumerate}
	where $\ell$ is the number of vertices met by both $X$ and $Y$.
	\label{mat:def:ksep}
\end{mydef}

We say that $\bg$ is \emph{vertically $k$-biconnected} if it admits no vertical $r$-biseparations for any $r<k$. We say that $\bg$ is \emph{simple} if it has no balanced circles of length 1 or 2 and no vertices incident to 2 or more unbalanced loops. A \emph{balancing set} of $\bg$ is an edge set $S$ such that $\bg\setminus S$ is balanced.

\begin{prop}[{\cite[Corollary 1.2]{slilaty2008}}]
	If $\bg$ is a connected and unbalanced biased graph on at least 3 vertices, then $G(\bg)$ is 2-connected if and only if $\Omega$ is vertically 2-biconnected and admits no balanced loops or balancing sets of rank 1.
	\label{mat:prop:2biconn}
\end{prop}

\begin{prop}[{\cite[Theorem 1.4]{slilaty2008}}]
	If $\bg$ is a connected and unbalanced biased graph on at least 3 vertices, then $G(\bg)$ is 3-connected if and only if $\bg$ is simple and vertically 3-biconnected and admits no balancing sets of rank 1 or 2.
	\label{mat:prop:slil}
\end{prop}

Let $\bo(N)$ be the biased graph obtained from $\bg(N)$ by adding an unbalanced loop to $v$. Call this loop $\eh$, so that $E(\bo(N)) = \eo$. Notice that $G(\bo(N)) = M(N)$. Thus to prove Theorem \ref{mat:thm:3connintro} it suffices to show that $\bo(N)$ satisfies the hypothesis of Proposition \ref{mat:prop:slil} if and only if $\g\setminus \B$ is connected and $\mg$ is 3-connected.

\begin{lem}
	The biased graph $\bo(N)$ is connected, unbalanced and simple.
	
	\begin{proof}
		Clearly $\bo(N)$ is connected because $\g$ is connected; and $\bo(N)$ is unbalanced because $\eh$ is unbalanced. It remains to show that $\bo(N)$ is simple. The only circle of $\bo(N)$ of length 1 is $\eh$, which is unbalanced. A balanced circle of length 2 would be a double edge in $\g$, which we have excluded by assumption. Hence $\bo(N)$ is simple.
	\end{proof}
\end{lem}

\begin{lem}
	If $\bo(N)$ admits a balancing set $S$ of rank 2, then $m=2$ and $S=\{\eh,e\}$ for some $e\in E$ such that $\g\setminus e$ contains no crossing.
	\begin{proof}
		A balancing set must contain $\eh$. Thus a balancing set of rank 2 is of the form $\{e,\eh\}$ for some $e\in E$ such that $\g\setminus e$ contains no crossing. This is only possible if $m=2$.
	\end{proof}
	\label{mat:lem:balancing}
\end{lem}

\begin{lem}
	No vertical $k$-biseparation of $\bo(N)$ satisfies condition (iii) of Definition \ref{mat:def:ksep}.
	
	\begin{proof}
		Given any partition of $\oe$, the part containing $\eh$ is unbalanced.
	\end{proof}
	\label{mat:lem:noiii}
\end{lem}
	
	Let $S_i$ be the vertex sets of the components of $\g\setminus \B$. For each $i$ let $T_i$ be the set of all edges meeting $S_i$. We call the $T_i$ the \emph{tracts} of $N$. Note that $\g\setminus \B$ is connected if and only if $E$ is the only tract of $N$. Also note that every vertex met by distinct tracts of $N$ is a boundary node. Since $\g$ is connected and $\B$ is an independent set, every tract meets at least 2 boundary nodes.
	
	A \emph{vertical $k$-separation} of a graph $\g$ is a partition $(X,Y)$ of $E$ such that $|X|,|Y|\geq k$ and exactly $k$ vertices are met by both $X$ and $Y$. Removing these $k$ vertices disconnects $\g$.
	
	\begin{lem}
		Let $(X,Y)$ be a partition of $\oe$ satisfying conditions (i) and (ii) of Definition \ref{mat:def:ksep} with $k=2$, and assume that $\eh\in X$. Then $(X,Y)$ satisfies (iv) if and only if there is a unique tract $T$ of $N$ containing $Y$ and satisfying one of
		\begin{enumerate}
			\item[(iv{$^\dagger$})] $(X\cap T,Y)$ is a vertical 1-separation of $\g(T)$ and $Y$ meets exactly one boundary node
			\item[(iv{$^\ddagger$})] $(X\cap T,Y)$ is a vertical 2-separation of $\g(T)$ and $Y$ meets no boundary nodes,
		\end{enumerate}
		where $\g(T)$ is the subgraph of $\g$ induced by $T$.
		\label{mat:lem:ivstar}
		
		\begin{proof}
			It is easy to verify that either of (iv$^\dagger$) or (iv$^\ddagger$) implies (iv). We prove the opposite direction. Suppose that $Y$ meets more than one boundary node. If $Y$ contains a tract of $N$, then $Y$ is balanced. If $Y$ does not contain a tract of $N$, then $|S|> 2$, where $S\subset (V\setminus\B) \cup v$ is the set of all vertices met by both $X$ and $Y$. In either case, $(X,Y)$ does not satisfy (iv).
			
			 Now suppose that $(X,Y)$ is a vertical 2-biseparation satisfying (iv), so that $Y$ meets at most one boundary node. Note that $Y$ must be contained in a tract $T$ of $N$, since otherwise $|S|>2$, a contradiction. Thus $S\cap V$ is the set of vertices of $\g(T)$ met by both $X\cap T$ and $Y$. Since $|S\cap V|$ is 2 minus the number of boundary nodes met by $Y$, $(X\cap T,Y)$ is a vertical $|S\cap V|$-separation of $\g(T)$.
		\end{proof}
	\end{lem}
	
\begin{lem}
	A partition $(X,Y)$ of $\oe$ satisfying conditions (i) and (ii) of Definition \ref{mat:def:ksep} with $k=2$ satisfies (v) if and only if it satisfies
	\begin{enumerate}
		\item[(v$^\dagger$)] $X\cap E$ and $Y\cap E$ are nonempty unions of tracts of $N$
	\end{enumerate}
	
	\begin{proof}
		It is easy to check that (v$^\dagger$) implies (v). We prove the opposite direction. If $Y$ is unbalanced, then it contains a path between distinct boundary boundary nodes. Thus if $\ell=1$, then $v$ is the only vertex of $\og$ met by both $X$ and $Y$. It follows that $Y$ is a nonempty union of tracts of $N$. The same follows for $X\setminus \eh= E\setminus Y$.
	\end{proof}
	
	\label{mat:lem:vstar}
\end{lem}
	
	\begin{proof}[{Proof of Theorem \ref{mat:thm:3connintro}}]
		The networks $N$ with $|V\setminus\B|=1$ are the star networks of Example \ref{mat:eg:star}. In this case the uniform matroid $M(N)=U_{2,|V|}$ is 3-connected by \cite[p. 312]{inukai1978}. Suppose that $|V\setminus\B|\geq 2$ for the remainder of the proof.
		
		We prove the ``only if'' direction first. Suppose that $M(N)$ is 3-connected. \emph{A fortiori} $M(N)$ is 2-connected, so $\mg$ is 2-connected by Theorem \ref{mat:thm:mainhyp}(iii). Suppose that $\mg\setminus \{i,j\}$ is disconnected for some $i,j\in V$. Condition (v$^\dagger$) of Lemma \ref{mat:lem:vstar} implies that there is only one tract of $N$, which must be $E$, so $\g\setminus \B$ is connected. If $i,j\in \B$, then $\g\setminus \B$ is disconnected, a contradiction. If $i,j\in \inte$ (resp., if $i\in \inte$ and $j\in \B$), then $\bo(N)$ admits a vertical 2-biseparation satisfying (iv$^\ddagger$) (resp., (iv$^\dagger$)) of Lemma \ref{mat:lem:ivstar} with $T=E$, a contradiction. Hence $\mg$ is 3-connected.
		
		Now we prove the ``if'' direction. Suppose that $\g\setminus \B$ is connected and $\mg$ is 3-connected. \emph{A fortiori} $\mg$ is 2-connected, so $\bo(N)$ is vertically 2-biconnected and admits no balancing sets of rank 1 by Theorem \ref{mat:thm:mainhyp}(iii) and Proposition \ref{mat:prop:2biconn}. If a balancing set of rank 2 existed, then Lemma \ref{mat:lem:balancing} would imply that $\g$ is not 2-connected and $m=2$. But then $\mg$ would not be 3-connected, a contradiction. Following Proposition \ref{mat:prop:slil}, it remains to show that $\bo(N)$ is vertically 3-biconnected. Suppose that $\bo(N)$ admits a vertical 2-biseparation $(X,Y)$. Lemma \ref{mat:lem:noiii} then says that $(X,Y)$ does not satisfy (iii). If $(X,Y)$ satisfies either (iv$^\dagger$) or (iv$^\ddagger$), then $\mg$ is not 3-connected, a contradiction. Specifically, in case (iv$^\dagger$), we can disconnect $\mg$ by removing the boundary node met by $Y$ and the vertex met by $X\setminus \eh$ and $Y$. In case (iv$^\ddagger$) we remove the two vertices met by both $X\setminus \eh$ and $Y$. Finally $(X,Y)$ cannot satisfy (v$^\dagger$) since $E$ is the only tract of $N$ by assumption.
	\end{proof}

Matroids that are 3-connected enjoy nice structural properties. For example, if the graphic matroid $M(\g)$ is 3-connected, then it is uniquely determined by $\g$ up to isomorphism. We have the following analog for Dirichlet matroids. Two networks $N=(\g,\B)$ and $N'=(\g',\B')$ are \emph{isomorphic} if there is an isomorphism of $\g$ and $\g'$ that maps $\B$ to $\B'$.

\begin{cor}
	If $\g\setminus \B$ is connected and $\mg$ is 3-connected, then up to isomorphism there are at most 27 networks $N'$ such that $M(N)\cong M(N')$.
	
	\begin{proof}
		This follows from Theorem \ref{mat:thm:3connintro}, Proposition \ref{mat:prop:balancing} and \cite[Corollary 2]{devos2018}.
	\end{proof}
\end{cor}

We say that the network $N$ is \emph{Hamiltonian} if there is a circuit of $M(N)$ meeting every vertex of $\og$. Such a circuit is called \emph{Hamiltonian}. For example, the star network $N$ from Example \ref{mat:eg:star} is Hamiltonian, and every circuit of $M(N)$ is Hamiltonian.

\begin{cor}
	If $N$ is Hamiltonian and
	\begin{equation}\frac{1}{3}|E|\geq |V|-|\B|+2,\end{equation}
	then for any Hamiltonian circuit $C$ of $M(N)$ there is a circle $C'\subset E$ disjoint from $C$ such that $(\g\setminus \B)\setminus C'$ is connected and $\mg\setminus C'$ is 3-connected.
	
	\begin{proof}
		This is an application of \cite[Theorem 6.1]{oxley2001} to Theorem \ref{mat:thm:3connintro}.
	\end{proof}
\end{cor}
